A Search for Supermassive Black Hole Binary Candidates in 46-Year Radio Light Curves of 83 Blazars

The combined University of Michigan Radio Astronomy Observatory (UMRAO) and Owens Valley Radio Observatory (OVRO) blazar monitoring programs at 14.5/15 GHz provide uninterrupted light curves of $\sim~46-50$ yr duration for 83 blazars, selected from amongst the brightest and most rapidly flaring blazars north of declination $-20^\circ$. In a search for supermassive black hole binary (SMBHB) candidates, we carried out tests for periodic variability using generalized Lomb-Scargle (GLS), weighted wavelet-Z (WWZ), and sine-wave fitting (SWF) analyses of this sample. We used simulations to test the effects of the power law spectrum of the power spectral density (PSD) on our findings, and show that the irregular sampling in the observed light curves has very little effect on the GLS spectra. Apparent periodicities and putative harmonics appear in all 83 of the GLS spectra of the blazars in our sample. We tested the reality of these apparent periodicities and harmonics with simulations, and found that in the overwhelming majority of cases they are due to the steep slope of the PSD, and should therefore be treated with great caution. We find one new SMBHB candidate: PKS 1309+1154, which exhibits a 17.9 year periodicity. The fraction of SMBHB candidates in our sample is $2.4_{-0.8}^{+3.2}\%$.

==> macros.tex <==
% MACROS.TEX contains generally useful macros, but not those specifically 
%            useful for paper formats.
%
\newcount\figureno  \newcount\tableno
\figureno=0         \tableno=0
%
\newbox\tablebox    \newdimen\tablewidth
%
\newbox\marginbox
\def\strutdepth{\dp\strutbox}
\def\strutheight{\ht\strutbox}
%
\def\smallformat{\hsize=5.5truein\hoffset=0.5truein
    \vsize=8truein\voffset=0.5truein\parskip=1pt}
\def\largeformat{\hsize=6.5truein\hoffset=0.0truein
    \vsize=8.5truein\voffset=0.0truein}
%
\newcount\sectionnumber \newcount\subsectionnumber 
\newcount\subsubsectionnumber
\sectionnumber=0 \subsectionnumber=0 \subsubsectionnumber=0
%
\def\secno{\ifcase\sectionnumber\or
     I\or II\or III\or IV\or V\or VI\or VII\or VIII\or IX\or
     X\or XI\or XII\fi}
\def\subsecno{\ifcase\subsectionnumber\or
     a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\fi}
\def\subsubsecno{\ifcase\subsubsectionnumber\or
     i\or ii\or iii\or iv\or v\or vi\or vii\or viii\or ix\or x\fi}
%
\def\section#1\par{\advance\sectionnumber by 1 \subsectionnumber=0
    \vskip 14pt plus 3pt minus 3pt\goodbreak
    \centerline{{\sc\secno.\ #1}}\nobreak\medskip}
\def\subsection#1\par{\advance\subsectionnumber by 1 \subsubsectionnumber=0
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\it\subsecno\/})\ {\it #1}}\nobreak\medskip}
\def\subsubsection#1\par{\advance\subsubsectionnumber by 1
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\eightrm\subsubsecno)}\ {\it #1}}\nobreak\medskip}
%
\def\today{\ifcase\month\or
    January\or February\or March\or April\or May\or June\or
    July\or August\or September\or October\or November\or December\fi
    \space\number\day, \number\year}
%
\def\sol{\ifmmode _{\mathord\odot}
         \else $_{\mathord\odot}$\fi}
\def\deg{\ifmmode ^{\circ}
         \else $^{\circ}$\fi}
\def\pdeg{\ifmmode $\setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}
          \else \setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}$\fi}
% Tony's definitions
\def\vs6{{\vskip 6pt \noindent}}
\def\vs15{{\vskip 15pt \noindent}}
%
\def\arcs{\ifmmode {^{\scriptscriptstyle\prime\prime}}
          \else $^{\scriptscriptstyle\prime\prime}$\fi}
\def\arcm{\ifmmode {^{\scriptscriptstyle\prime}}
          \else $^{\scriptscriptstyle\prime}$\fi}
\newdimen\sa  \newdimen\sb
\def\parcs{\sa=.07em \sb=.03em
     \ifmmode $\rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa$
     \else \rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa\fi}
\def\parcm{\sa=.08em \sb=.03em
     \ifmmode $\rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb$
     \else \rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb\fi}
%
\def\s#1{{\sc #1}}
\def\et{\hbox{\it et al.}}
\def\ET{{\it ET AL.}}
\def\expo#1{\ifmmode \times 10^{#1}
            \else $\times 10^{#1}$\fi}
\def\page{\vfill\eject}
\def\leaderfil{\leaders\hbox to 5pt{\hss.\hss}\hfil}
%
\def\mo{\ifmmode ^{-1}
        \else $^{-1}$\fi}
\def\sup#1{$^{\rm #1}$}
\def\mag{\sup{m}}
\def\muK{\,$\mu$\hbox{K}}
\def\,{\thinspace}
\def\tc#1{3C\,#1}
\def\dots{\relax\ifmmode \ldots
          \else $\ldots$\fi}
\def\WHzsr{\ifmmode $W\,Hz\mo\,sr\mo$
           \else W\,Hz\mo\,sr\mo \fi}
\def\mKs{\ifmmode $\,mK\,s$^{-1/2} 
         \else \,mK\,s$^{-1/2}$ \fi}
\def\microns{\ifmmode \,\mu$m$
             \else \,$\mu$m\fi}
\def\micron{\microns}

%
\def\gsim{\lower.6ex\hbox{$\buildrel>\over\sim$}}
\def\lsim{\lower.6ex\hbox{$\buildrel<\over\sim$}}
\def\ra[#1 #2 #3.#4]{#1\sup{h}#2\sup{m}#3\sup{s}\llap.#4}
\def\dec[#1 #2 #3.#4]{#1\deg#2\arcm#3\arcs\llap.#4}
\def\deco[#1 #2 #3]{#1\deg#2\arcm#3\arcs}
%
\def\refindent{\hangindent=1em \hangafter=1 \noindent}
\def\ref #1;#2;#3;#4\par{\refindent #1,{\it #2},{\bf #3},#4.\par}
\def\ajref #1;#2;#3;#4\par{\refindent #1. #2 {\bf #3},#4.\par}
\def\vref #1\par{\refindent #1.\par}
\def\cref #1;#2;#3;#4;#5\par{\refindent #1, in{\it #2}, 
                             \hbox{ed.}#3 #4, \hbox{p.} #5.\par} 
\def\bref #1;#2;#3\par{\refindent #1, {\it #2} (#3).\par}
%
%
\def\tabl #1\par{\centerline{TABLE \number\tableno}
                 \vskip 7pt
                 \centerline{#1}\nointerlineskip\noindent}
\def\endtable{\tablewidth=\wd\tablebox 
    $$\hss\copy\tablebox\hss$$
    \vskip-\lastskip\vskip -2pt}
\def\tablenote#1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=\parindent \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotenoindent #1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=0pt \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotes #1\par{
            \iftform \goodbreak\topinsert{
                 \centerline{NOTES TO TABLE \number\tableno}
                 \vskip .3cm\noindent
                 \eightpoint\input #1 }\endinsert
            \else \iftabsopen\relax
                  \else\immediate\openout\tabs=junk1\tabsopentrue\fi
                \vskip .5cm
                \centerline{NOTES TO TABLE \number\tableno} \vskip .5cm
                \immediate\write\tabs{\string\etable\space#1\string\par}
            \fi}
\def\doubleline{\vskip 3pt\hrule \vskip 1.5pt \hrule \vskip 5pt}
%
% macros for marginal stuff
%
\def\marginstuff#1{\setbox\marginbox=\vtop{
    \hsize=60pt\tolerance=10000\hbadness=10000
%    \hsize=70pt\tolerance=10000\hbadness=10000
    \parindent=0pt\eightpoint#1\par}\strut}
\def\setmarginal{\strut\vadjust{\kern-\strutdepth\kern-\ht\marginbox\vtop{%
    \moveleft 70pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%    \moveleft 80pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%
% macro for absolute positioning on a page
%
\newdimen\offset 
\newdimen\unita \newdimen\unitb
\newdimen\mina  \newdimen\minb 
%
\unita=1.0cm \mina=0.0cm
\unitb=1.0in \minb=0.0in
%
%
\def\point #1 #2 #3;{\offset=#1\unitb\advance\offset by \minb%
    \rlap{\lower\offset\hbox{\hglue #2\unitb #3}}}%
%
% macros for memos
%
\font\ssq=cmssq8 at 7pt \font\ssbx=cmssbx10 at 12pt 
\setbox0=\hbox{\ssq ATENDEES \rm\quad}
\newdimen\atndwd \atndwd=\wd0
\def\file{}
\def\memo{\hsize=5.875in \hoffset=0.3125in
    \vsize=9in     \voffset=0in
    \elevenpoint
    \vglue -0.8in
    \line{\ssq\hfil INTEROFFICE MEMORANDUM\hfil \llap{\twelvepoint\bf\file}}
    \vskip 10pt
    \centerline{\hbox to 5.4in{\ssbx C A L I F O R N I A\hskip 12pt
                I N S T I T U T E\hskip 12pt O F\hskip 12pt 
                T E C H N O L O G Y}}
    \vskip 30pt}
\def\to#1{\line{\ssq TO \rm\quad #1\hfil\today}
          \vskip 12pt}
\def\from#1{\line{\ssq FROM \rm\quad C. R. Lawrence#1\hfil
                  \ssq EXTENSION \rm\quad 4976\quad\quad
                  \ssq MAIL CODE \rm\quad 105-24}
            \vskip 12pt}
\def\subject#1{\line{\ssq SUBJECT \rm\quad#1\hfil}
               \vskip 12pt}
\def\attendees#1{\hangindent=\atndwd \hangafter=1 \noindent
                \ssq ATENDEES \rm\quad#1
                \vskip 24pt}
\def\OVRO#1{\def\file{OVRO 5m \rlap{#1-87}}}

